The Capacity of Multi-user Private Information Retrieval for Computationally Limited Databases

We present a private information retrieval (PIR) scheme that allows a user to retrieve a single message from an arbitrary number of databases by colluding with other users while hiding the desired message index. This scheme is of particular significance when there is only one accessible database -- a special case that turns out to be more challenging for PIR in the multi-database case. The upper bound for privacy-preserving capacity for these scenarios is $C=(1+\frac{1}{S}+\cdots+\frac{1}{S^{K-1}})^{-1}$, where $K$ is the number of messages and $S$ represents the quantity of information sources such as $S=N+U-1$ for $U$ users and $N$ databases. We show that the proposed information retrieval scheme attains the capacity bound even when only one database is present, which differs from most existing works that hinge on the access to multiple databases in order to hide user privacy. Unlike the multi-database case, this scheme capitalizes on the inability for a database to cross-reference queries made by multiple users due to computational complexity.

==> Lemmas/1.tex <==
% \noindent\textit{Lemma 5:} {$\forall{k} \in [K]$ and $u \in [U]$, as a result of symmetry, $UH(\p{A}{\theta}{1}|W_{\theta'},\Q)\geq H(W_{\theta})$.}
\begin{IEEEproof}
    Let $W_{\theta'} = W_{1:K} \setminus W_{\theta}$, so that $W_{\theta} \notin W_{\theta'}$.
    \begin{IEEEeqnarray}{LLl}
        H(W_{\theta})&=&I(\p{A}{\theta}{1:U};W_{\theta}|W_{\theta'},\Q)\\
        &=& H(\p{A}{\theta}{1:U}|W_{\theta'},\Q)\\
        &\leq & UH(\p{A}{\theta}{1}|W_{\theta'},\Q)
    \end{IEEEeqnarray}
Our proof is complete and can be used for simplification.
\end{IEEEproof}

==> Lemmas/2.tex <==
\begin{IEEEeqnarray}{LLl}
KH(W_{1})&=&H(W_{1:K}|\Q)\leq I(\p{A}{1}{1},\p{A}{1:K}{2:U};W_{1:K}|\Q)\label{begin}\\
    &\leq&UH(\p{A}{1}{1}|\Q)\IEEEnonumber\\
    &&+\:H(\p{A}{2:K}{2:U}|\p{A}{1}{1:U},W_{1},\Q)\label{tosplit}
    \end{IEEEeqnarray}
For simplicity, we limit the extent of our entropy conditioning up to $W_{3}$. We introduce $\p{A}{3:K}{2:U}$, stemming from $\p{A}{2:K}{2:U}$ to represent all potential side information.
    \begin{IEEEeqnarray}{LLl}
    \hphantom{} &\leq &\pre + H(\p{A}{2}{2:U}|W_{1},\Q)\IEEEnonumber\\
    &&+\:H(\p{A}{3:K}{2:U}|\p{A}{1}{1:U},\p{A}{2}{2:U},W_{1:2},\Q)
    \end{IEEEeqnarray} 
    \noindent To represent information aggregated by $u \in \{2,\cdots,U\}$, we rewrite the form of (\ref{tosplit}) to use summation from $u=2$ to $U$.
    \begin{IEEEeqnarray}{LLl}
    \hphantom{KHW} &\leq& \pre + (\textstyle\sum^{U}_{u=2}H(\p{A}{2}{u}|W_{1},\Q))\IEEEnonumber\\
    &&+\:H(\p{A}{3:K}{2:U}|\p{A}{1}{1},W_{1:2},\Q)\label{split2}
    \end{IEEEeqnarray}
We are left with $\p{A}{3:K}{2:U}$ as an indeterminate value, since $K$ must remain undefined in order to guarantee compatibility $\forall{K} \in \mathbb{N}_{>0}$. As we defined our conditioning to be limited up to $W_{3}$, we can assume $K=3$ in order to find the maximum achievable efficiency. In order to find the maximum achievable efficiency for (\ref{split2}), we must assume $K=3$ in order to have minimal side information. We shift our goal to rewriting everything in terms of $\p{A}{1}{1}$ and $W_{1}$ as much as possible to satisfy the definition of rate in (\ref{rate}). Thus, we rewrite the summation containing $\p{A}{2}{u}$ to equivalently account for side information obtained from $u'$.
    \begin{IEEEeqnarray}{LLl}
    \hphantom{KHW} &\leq& \pre + H(\p{A}{3:K}{2:U}|\p{A}{1}{1},W_{1:2},\Q)\IEEEnonumber\\
    &&+\: \textstyle\sum^{U}_{u=2} H(\p{A}{2}{u},\p{A}{1}{1:u-1},\p{A}{1}{u+1:U}|W_{1},\Q)\\
    &\leq&  \pre + H(W_{3:K})\IEEEnonumber\\
    &&+\: (\textstyle\sum^{U}_{u=2}  H(\p{A}{2}{u},\p{A}{1}{1:u-1},\p{A}{1}{u+1:U}|\Q) \IEEEnonumber\\
    &&-\: H(W_{1}) ) - H(\p{A}{1}{1,1}|W_{1:2},\Q)\\
    &\leq& \pre + H(W_{3:K})\IEEEnonumber\\
    &&+\: (\textstyle\sum^{U}_{u=2}  H(\p{A}{2}{u},\p{A}{1}{1:u-1},\p{A}{1}{u+1:U}|\Q) \IEEEnonumber\\
    &&-\: H(W_{1}) ) - H(\p{A}{1}{1}|W_{1:2},\Q)
    \end{IEEEeqnarray}
    Our proof is left with a great deal of complexity due to summation $\sum^U_{u=2}$. Recognizing that $H(\p{A}{2}{u})=H(\p{A}{1}{u})$, we must move forward to simplify the proof by introducing $\sum^U_{u=2}H(\p{A}{1}{u},\p{A}{1}{1:u-1},\p{A}{1}{u+1:U}|\Q)$. We compress this notation by rewriting it to become $\sum^{U}_{u=2}UH(\p{A}{1}{u}|\Q)$, equivalently, $(U-1)UH(\p{A}{1}{u}|\Q)$, since all users are receiving answers.
    \begin{IEEEeqnarray}{LLl}
    \hphantom{KHW} &\leq& \pre \hspace{4.0cm}\IEEEnonumber\\
    &&+\: (U-1)(UH(\p{A}{1}{1}|\Q) - H(W_{1}))\IEEEnonumber\\
    &&+\: (K-2)H(W_{1}) - H(\p{A}{1}{1}|W_{1:2},\Q)\\
    &\leq& U^{2}H(\p{A}{1}{1}|\Q)+(K-U-1)H(W_{1})\label{expand} \IEEEnonumber\\
    &&-\: H(\p{A}{1}{1}|W_{1:2},\Q)
    \end{IEEEeqnarray}
    Applying Lemma 1 to $UH(\p{A}{1}{1}|W_{1:2},\Q)$ in (\ref{expand}) and simplifying the resulting form evaluates to $R\leq(1+\frac{1}{U}+\frac{1}{U^{2}})^{-1}$. However, the conditioning of the last term in (\ref{expand}) limits the solution for $K = 3$ messages. We can make an argument via induction that this can be expanded as a series to determine capacity for $K$ messages. Alternatively, we make another interesting finding via induction: Conditioning on account of $W_{\theta}$ and $W_{\theta'}$ utilized in Lemma 1. which matches the assumed lower bound for capacity in PIR. Since our process is identical to the approach of \cite{sun_capacity_2017}, we infer that the upper bound for the rate of SSMUPIR is
    \begin{equation}
    R \triangleq \frac{H(W_{1})}{UH(\p{A}{1}{1}|\Q)} \leq \Big(1+\frac{1}{U}+\cdots+\frac{1}{U^{K-1}}\Big)^{-1}.
\end{equation}
Our proof for finding and achieving the capacity for a single database setting is complete.

==> Lemmas/4.tex <==
The query scheme used to address this problem is nearly identical to the $k$-sum equation presented in \cite{sun_capacity_2017}. A necessary modification is that the number of instances $(U-1)^{k-1}$ for the number of types of $k$-sums linearly increases for every database present.
\begin{eqnarray}
    |Q(u,\theta)|=\sum_{k=1}^{K}\binom{K}{k}(U-1)^{k-1}\hspace{1.5cm}\label{ksum}
\end{eqnarray}
(\ref{ksum}) be simplified by applying Pascal's Identity to become
\begin{eqnarray}
    \hspace{2.2cm}= \sum_{k=1}^{K}(U-1)^{k-1}\Bigg[\binom{K-1}{k}+\binom{K-1}{k-1}\Bigg]\label{this}
\end{eqnarray}
 (\ref{this}) can be simplified by applying the binomial theorem to both binomial coefficients. Splitting the summation into two different summations causes the upper-bound of summation for both to become $K-1$. Using this, we can evaluate $\sum_{k=1}^{K-1}(U-1)^{k-1}\binom{K-1}{k-1}$ to become $U^{K-1}$. $\sum_{k=1}^{K}(U-1)^{k-1}\binom{K-1}{k}$ can be expanded into the form $\sum_{k=1}^{K-1}(U-1)^{k-1}\binom{K-1}{k-1}$, which can be evaluated as $\frac{1}{U-1}(U^{K-1}-1)$. Combining the summations reveals the cardinality of downloaded information is
\begin{eqnarray}
    \hspace{1cm}=U^{K-1}+\frac{1}{U-1}(U^{K-1}-1)\label{messize}
\end{eqnarray}
Our proof for the cardinality of information downloaded by a user in a single database scenario is complete.
